Dual-Primal Isogeometric Tearing and Interconnecting solvers for multipatch dG-IgA equations

In this paper we consider a new version of the dual-primal isogeometric tearing and interconnecting (IETI-DP) method for solving large-scale linear systems of algebraic equations arising from discontinuous Galerkin (dG) isogeometric analysis of diffusion problems on multipatch domains with non-matching meshes. The dG formulation is used to couple the local problems across patch interfaces. The purpose of this paper is to present this new method and provide numerical examples indicating a polylogarithmic condition number bound for the preconditioned system and showing an incredible robustness with respect to large jumps in the diffusion coefficient across the interfaces.

==> Makros.tex <==

  \usepackage{xifthen}% provides \isempty test

  \newcommand{\genref}[2]{#2\,\ref{#1}}
 
  \newcommand{\thmref}[1]{\genref{#1}{Theorem}}
  \newcommand{\lemref}[1]{\genref{#1}{Lemma}}
  \newcommand{\defref}[1]{\genref{#1}{Definition}}
  \newcommand{\assref}[1]{\genref{#1}{Assumption}}
  \newcommand{\propref}[1]{\genref{#1}{Proposition}}
  \newcommand{\corref}[1]{\genref{#1}{Corrolary}}
  \newcommand{\equref}[1]{(\ref{#1})} 
  \newcommand{\secref}[1]{Section\,\ref{#1}}
  \newcommand{\tabref}[1]{Table\,\ref{#1}}
  \newcommand{\figref}[1]{Figure\,\ref{#1}}
 
 \newcommand{\mc}[3]{\multicolumn{#1}{#2}{#3}}
 
  \newcommand{\MatThree}[9]
  {
    \begin{bmatrix}
    #1 & #2 & #3\\
    #4 & #5 & #6\\
    #7 & #8 & #9
    \end{bmatrix}
  }
  
  \newcommand{\MatTwo}[4]
  {\begin{bmatrix}
    #1 & #2\\
    #3 & #4
  \end{bmatrix}}
  
  \newcommand{\VecTwo}[2]
  {\begin{bmatrix}
    #1 \\
    #2 
  \end{bmatrix}}
  \newcommand{\VecThree}[3]
  {\begin{bmatrix}
    #1 \\
    #2 \\
    #3
  \end{bmatrix}}
  

  \newcommand{\DN}[1]{\frac{\partial #1}{\partial n}}
  \newcommand{\dd}[2]{\frac{\partial #1}{\partial #2}}
  \newcommand{\real}[1][]
  {
    \ifthenelse{\isempty{#1}}%
    {\mathbb{R}}
    {\mathbb{R}^{{#1}}}
  }
    \newcommand{\nat}[1][]
  {
    \ifthenelse{\isempty{#1}}%
    {\mathbb{N}}
    {\mathbb{N}^{#1}}
  }
  \DeclareMathOperator{\mdiv}{div}
  \DeclareMathOperator{\grad}{\nabla}
  \renewcommand{\ker}[1]{\text{ker}(#1)}
    \newcommand{\supp}{\text{supp}}
    \newcommand{\spn}{\text{span}}
    \newcommand{\lanO}[1]{\mathcal{O}\left(#1\right)}
    \newcommand{\diam}{\text{diam}}
    \newcommand{\for}{\mbox{for }}
    \newcommand{\range}[1]{\mathcal{R}(#1)}
   
   
  \newcommand{\onB}[3][]
  {
  \ifthenelse{\isempty{#1}}%
    {#2_{h|\partial \gDom\sMP[#3]}}
    {#2_{#1|\partial \gDom\sMP[#3]}}
  }
  \newcommand{\uOnB}[1]{\onB{u}{#1}}
  \newcommand{\vOnB}[1]{\onB{v}{#1}}
  
  \newcommand{\bil}[3][]
  {
  \ifthenelse{\isempty{#1}}%
    {a(#2,#3)}
    {a\sMP[#1](#2,#3)}
  }
  \newcommand{\func}[3][]
  {
  \ifthenelse{\isempty{#1}}%
    {\left\langle #2, #3 \right\rangle}
    {\left\langle #2\sMP[#1], #3 \right\rangle}
  }
  
  \newcommand{\mat}[1]{\boldsymbol{#1}}
  \renewcommand{\vec}[1]{\boldsymbol{#1}}
  
  \newcommand{\LTwoNorm}[2]{\left\|#1\right\|_{L^2(#2)}}
  \newcommand{\LInfNorm}[2]{\left\|#1\right\|_{L^\infty(#2)}}
  \newcommand{\HNorm}[3]{\left\|#2\right\|_{H^{#1}(#3)} }
  \newcommand{\HOneNorm}[2]{\HNorm{1}{#1}{#2}}
  \newcommand{\HSNorm}[3]{\left\|#2\left\|_{H^{#1}(#3)}}
  \newcommand{\HOneSNorm}[2]{\HSNorm{1}{#1}{#2}}
  \newcommand{\dGnorm}[1]{\left\|#1\right\|_{dG}}
  
  
  \newcommand{\DiscLLocNorm}[2]{|#1|_{#2}}
  \newcommand{\DiscLNorm}[1]{|#1|_{\Square}}
  \newcommand{\DiscHNorm}[1]{|#1|_{\nabla}}
  
  \newcommand{\RealSNorm}[1]{\left\|\!\left|#1\right\|\!\right|_{\nabla}}
  \newcommand{\RealTNorm}[1]{\left\|\!\left|#1\right\|\!\right|_{e}}
    
%%% IGA %%%%
\newcommand{\x}[1][]{\ifthenelse{\isempty{#1}}{x}{x_{#1}}}

\newcommand{\g}[1]{\gBSplFormat{#1}}

\newcommand{\pDim}{{d}}
\newcommand{\gDim}{g}
\newcommand{\pDom}[1][]{\ifthenelse{\isempty{#1}}{(0,1)^\pDim}{\ifthenelse{\equal{#1}{2}}{[0,1]^2}{(0,1)^\pDim}}}
\newcommand{\gDom}{\Omega}

\newcommand{\intBaseLetter}{\Gamma}
\newcommand{\gIntG}[2]{\intBaseLetter^{(#1,#2)}}
\newcommand{\gInt}{\gIntG{k}{l}}
\newcommand{\gIntMP}{\intBaseLetter}
\newcommand{\gIntS}{\intBaseLetter_S}
\newcommand{\pInt}{\pBaseFormat{\intBaseLetter}}

\newcommand{\nMP}{N}
\newcommand{\iMP}{{k}}
\newcommand{\sMP}[1][]{\ifthenelse{\isempty{#1}}{^{(\iMP)}}{^{(#1)}}}
\newcommand{\ext}{_e}

\newcommand{\iSet}{{\mathcal{I}}}
\newcommand{\iSetMesh}{\iSet_{\pMeshBase}}
\newcommand{\piSet}{{\mathcal{\pBaseFormat{I}}}}
\newcommand{\ifSet}{\iSet_{\mathcal{F}}}
\newcommand{\eSet}{{\mathcal{E}}}
\newcommand{\fSet}{{\mathcal{F}}}
\newcommand{\vSet}{{\mathcal{V}}}

\newcommand{\iVar}{\iota}

\newcommand{\kn}[1][]{\ifthenelse{\isempty{#1}}{\xi}{\xi_{#1}}}
\newcommand{\knV}{\Xi}
\newcommand{\nkn}{m}
\newcommand{\ncoef}{n}
\newcommand{\nIntKnotspan}{\nu}
\renewcommand{\deg}{p}
\newcommand{\mul}{r}
\newcommand{\IndexSet}{\mathcal{B}}


\newcommand{\BSplBaseLetter}{N}
\newcommand{\gBSplFormat}[1]{\check{#1}}
\newcommand{\gBSplBaseLetter}{\gBSplFormat{\BSplBaseLetter}}

\newcommand{\BSplG}[2]{\BSplBaseLetter_{#1,#2}}
\newcommand{\BSpl}{\BSplG{i}{\deg}}
\newcommand{\BSplFamG}[2]{\{\BSplG{#1}{#2}\}_{#1\in\iSet}}%_{#1=1}^{#3}}
\newcommand{\BSplFam}{\BSplFamG{i}{\deg}}%{\pDim}}

\newcommand{\gBSplG}[2]{\gBSplBaseLetter_{#1,#2}}
\newcommand{\gBSpl}{\gBSplG{i}{\deg}}
\newcommand{\gBSplFamG}[3][]{\ifthenelse{\isempty{#1}}
{\{\gBSplG{#2}{#3}\}_{#2\in\iSet}}
{\{\gBSplG{#2}{#3}\sMP[#1]\}_{#2\in\iSet\sMP[#1]}}}%_{#1=1}^{#3}}

\newcommand{\gBSplFam}{\gBSplFamG{i}{\deg}}%{\pDim}}
\newcommand{\nBasis}{M}

\newcommand{\pBaseFormat}[1]{\hat{#1}}
\newcommand{\meshBaseLetter}{Q}
\newcommand{\meshBaseFormat}{\mathcal{\meshBaseLetter}}
\newcommand{\pMeshBase}{\pBaseFormat{\meshBaseFormat}}
\newcommand{\pMesh}{\pMeshBase_h}
\newcommand{\gMesh}{\meshBaseFormat_h}
\newcommand{\gCell}[1][]{\ifthenelse{\isempty{#1}}{\meshBaseLetter}{\meshBaseLetter_{#1}}}
\newcommand{\pCell}[1][]{\ifthenelse{\isempty{#1}}{\pBaseFormat{\meshBaseLetter}}{\pBaseFormat{\meshBaseLetter}_{#1}}}

\newcommand{\Cp}[1][]{\ifthenelse{\isempty{#1}}{P_{i}}{P_{#1}}}
\newcommand{\geoMap}{G}

\newcommand{\baseV}{V}

\newcommand{\genSp}[3][]{\ifthenelse{\isempty{#1}}{#2_{#3}}{#2_{#3,#1}}}
\newcommand{\gVh}{\genSp{\baseV}{h}}
\newcommand{\gVhe}{\genSp[e]{\baseV}{h}}
\newcommand{\ghVhe}{\genSp[e]{\ContSpaceFormat{\baseV}}{h}}
\newcommand{\pVh}{\genSp{\mathrm S}{h}}
\newcommand{\gVB}{\genSp[h]{\baseV}{\Gamma}}
\newcommand{\gVBe}{\genSp[h]{\baseV}{\Gamma\ext}}
\newcommand{\gVI}{\genSp[h]{\baseV}{I}}

\newcommand{\VD}[1][]{\genSp[#1]{\baseV}{D}}
\newcommand{\VO}[1][]{\genSp[#1]{\baseV}{0}}
\newcommand{\VDh}{\VD[h]}
\newcommand{\VOh}{\VO[h]}

\newcommand{\dualBasis}[1]{\lambda_{i,\deg}\left(#1\right)}

%%% IETI %%%%
\newcommand{\genLocSpace}[3][]{\ifthenelse{\isempty{#1}}{#2_{#3}}{#2_{#3}\sMP[#1]}}
\newcommand{\IntermSpaceForamt}[1]{\widetilde{#1}}
\newcommand{\ContSpaceFormat}[1]{\widehat{#1}}

\newcommand{\base}{W}
\newcommand{\hW}{\ContSpaceFormat{\base}}
\newcommand{\tW}{\IntermSpaceForamt{\base}}

\newcommand{\sB}{_B}
\newcommand{\sBe}{_{B_e}}
\newcommand{\sI}{_I}

\newcommand{\setB}{\iSet\sB} %\Theta
\newcommand{\setI}{\iSet\sI} %\Theta
  
  \newcommand{\emb}{\IntermSpaceForamt{I}}
  \newcommand{\tB}{\IntermSpaceForamt{B}}
  \newcommand{\tg}{\IntermSpaceForamt{g}}
  \newcommand{\tphi}{\IntermSpaceForamt{\phi}}
  \newcommand{\nLag}{\Lambda}
  \newcommand{\LamSet}{U}
  \newcommand{\tLamSet}{\IntermSpaceForamt{U}}

 \newcommand{\LocVB}[1][]{\ifthenelse{\isempty{#1}}{\base}{\ifthenelse{\equal{#1}{L}}{\overline{\base}}{\base\sMP[#1]}}}
  \newcommand{\Wp}[1][]{\genLocSpace[#1]{\base}{\Pi}}     
  \newcommand{\Wd}[1][]{\genLocSpace[#1]{\base}{\Delta}}  
  \newcommand{\tWp}[1][]{\genLocSpace[#1]{\tW}{\Pi}}
  \newcommand{\tWd}[1][]{\genLocSpace[#1]{\tW}{\Delta}}

  
  
 \newcommand{\GenOp}[2][]{
  \ifthenelse{\isempty{#1}}
    {#2}
    {#2\sMP[#1]}
  }

  \newcommand{\Sop}[1][]{\GenOp[#1]{S}}
  \newcommand{\tSop}[1][]{\IntermSpaceForamt{\Sop{#1}}} 
  \newcommand{\Nop}[1][]{\GenOp[#1]{N}}
  \newcommand{\Kop}[1][]{\GenOp[#1]{K}}
  \newcommand{\Ci}[1][]{\GenOp[#1]{C}}
  
  \newcommand{\np}[1][]{ \ifthenelse{\isempty{#1}} {n_{\Pi}} {n_{\Pi}\sMP[#1]} }
  
  \newcommand{\GenMatXX}[3][]
  {
  \ifthenelse{\isempty{#1}}%
    {#2_{#3}}
    {#2_{#3}\sMP[#1]}
  }
  
  
  \newcommand{\KBB}[1][]{ \GenMatXX[#1]{\Kb}{BB}}
  \newcommand{\KIB}[1][]{ \GenMatXX[#1]{\Kb}{IB}}
  \newcommand{\KBI}[1][]{ \GenMatXX[#1]{\Kb}{BI}}  
  \newcommand{\KII}[1][]{ \GenMatXX[#1]{\Kb}{II}}
  
  \newcommand{\KBBop}[1][]{ \GenMatXX[#1]{\Kop}{BB}}
  \newcommand{\KIBop}[1][]{ \GenMatXX[#1]{\Kop}{IB}}
  \newcommand{\KBIop}[1][]{ \GenMatXX[#1]{\Kop}{BI}}  
  \newcommand{\KIIop}[1][]{ \GenMatXX[#1]{\Kop}{II}}
  
  \newcommand{\SPP}[1][]{ \GenMatXX[#1]{\Sb}{\Pi\Pi}}
  \newcommand{\SDP}[1][]{ \GenMatXX[#1]{\Sb}{\Delta\Pi}}
  \newcommand{\SPD}[1][]{ \GenMatXX[#1]{\Sb}{\Pi\Delta}}
  \newcommand{\SDD}[1][]{ \GenMatXX[#1]{\Sb}{\Delta\Delta}}
  
  \newcommand{\SPPop}[1][]{ \GenMatXX[#1]{\Sop}{\Pi\Pi}}
  \newcommand{\SDPop}[1][]{ \GenMatXX[#1]{\Sop}{\Delta\Pi}}
  \newcommand{\SPDop}[1][]{ \GenMatXX[#1]{\Sop}{\Pi\Delta}}
  \newcommand{\SDDop}[1][]{ \GenMatXX[#1]{\Sop}{\Delta\Delta}}
  

  \newcommand{\RestrBD}[1][]{ \GenMatXX[#1]{{R}}{B\Delta}}
  \newcommand{\RestrBP}[1][]{ \GenMatXX[#1]{{R}}{B\Pi}}
  \newcommand{\RestrD}[1][]{ \GenMatXX[#1]{{R}}{\Delta}}  
  \newcommand{\RestrP}[1][]{ \GenMatXX[#1]{{R}}{\Pi}}
  
  \newcommand{\RestrScB}[1][]{ \GenMatXX[#1]{{R}}{D,B}}
  \newcommand{\RestrScD}[1][]{ \GenMatXX[#1]{{R}}{D,\Delta}}
     
  \newcommand{\wP}[1][]
  {
    \ifthenelse{\isempty{#1}}%
    {\boldsymbol{w}_{\Pi}}
    {\boldsymbol{w}_{\Pi}\sMP[#1]}
  }

  \newcommand{\wD}[1][]
  {
    \ifthenelse{\isempty{#1}}%
    {w_{\Delta}}
    {w_{\Delta}\sMP[#1]}
  }
  \newcommand{\fP}[1][]
  {
    \ifthenelse{\isempty{#1}}%
    {\boldsymbol{f}_{\Pi}}
    {\boldsymbol{f}_{\Pi}\sMP[#1]}
  }
  \newcommand{\fD}[1][]
  {
    \ifthenelse{\isempty{#1}}%
    {f_{\Delta}}
    {f_{\Delta}\sMP[#1]}
  }
  

  %\newcommand{\uI}{u_I}
  %\newcommand{\uB}{u_B}

  \newcommand{\Scal}[1][]{  \ifthenelse{\isempty{#1}}{{\delta^{\dagger}}}{{\delta_{#1}^{\dagger}}}}
  
  \newcommand{\DHE}[1][]{  \ifthenelse{\isempty{#1}}{\mathcal{H}}{\mathcal{H}\left(#1\right)}}
  %\newcommand{\DHEloc}[1][]{  \ifthenelse{\isempty{#1}}{\mathcal{H}_{loc}}{\mathcal{H}_{loc}\left(#1\right)}}
  \newcommand{\DHEreal}[1][]{  \ifthenelse{\isempty{#1}}{\mathcal{H}_{\mathcal{Q}_1}}{\mathcal{H}_{\mathcal{Q}_1}\left(#1\right)}}
  
  %%%%%%%%%%% matrices and vectors %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newcommand{\tmu}{\IntermSpaceForamt{\boldsymbol{\mu}}} 
 \newcommand{\tBb}{\IntermSpaceForamt{\boldsymbol{B}}} 
 \newcommand{\tgb}{\IntermSpaceForamt{\boldsymbol{g}}}
 \newcommand{\tSb}[1][]{\IntermSpaceForamt{\Sb{#1}}}
 
 \newcommand{\Pvec}{\boldsymbol{P}} % control points
 \newcommand{\Fb}{\boldsymbol{F}} 
 \newcommand{\Bb}{\boldsymbol{B}}
 \newcommand{\db}{\boldsymbol{d}}
 \newcommand{\gb}{\boldsymbol{g}}
 \newcommand{\lambdavec}{\boldsymbol{\lambda}}
 \newcommand{\xvec}{\boldsymbol{x}}
 \newcommand{\xivec}{\boldsymbol{\xi}}
 \newcommand{\phivec}{\boldsymbol{\phi}}
 \newcommand{\nvec}{\boldsymbol{n}} % outer unit normal vector
 \newcommand{\evec}{\boldsymbol{e}}

 
 \newcommand{\GenBold}[2][]{
  \ifthenelse{\isempty{#1}}
    {\boldsymbol{#2}}
    {\boldsymbol{#2}\sMP[#1]}
  }
  \newcommand{\GenBoldUnderscore}[3][]{
  \ifthenelse{\isempty{#1}}
    {\boldsymbol{#2}#3}
    {\boldsymbol{#2}#3\sMP[#1]}
  }
  
 \newcommand{\Ib}{\GenBold{I}}
 
 \newcommand{\ub}[1][] {\GenBold[#1]{u}}
 \newcommand{\wb}[1][] {\GenBold[#1]{w}}
 \newcommand{\vb}[1][] {\GenBold[#1]{v}}  
 \newcommand{\Nb}[1][] {\GenBold[#1]{N}}
  
 \newcommand{\gvec}[1][]  {\GenBold[#1]{g}}
 \newcommand{\fvec}[1][]  {\GenBold[#1]{f}}
 \newcommand{\Kb}[1][]    {\GenBold[#1]{K}}
 \newcommand{\Sb}[1][]    {\GenBold[#1]{S}}
  
  
  \newcommand{\fvecB}[1][] {\GenBoldUnderscore[#1]{f}{\sB} }
  \newcommand{\fvecI}[1][] {\GenBoldUnderscore[#1]{f}{\sI} }
  \newcommand{\IbB}[1][]  {\GenBoldUnderscore[#1]{\Ib}{\sB} }
  \newcommand{\uIb}[1][] {\GenBoldUnderscore[#1]{u}{\sI} }
  \newcommand{\uBb}[1][] {\GenBoldUnderscore[#1]{u}{\sB} }


